A mathematical model for the within-host (re)infection dynamics of SARS-CoV-2

Interactions between SARS-CoV-2 and the immune system during infection are complex. However, understanding the within-host SARS-CoV-2 dynamics is of enormous importance, especially when it comes to assessing treatment options. Mathematical models have been developed to describe the within-host SARS-CoV-2 dynamics and to dissect the mechanisms underlying COVID-19 pathogenesis. Current mathematical models focus on the acute infection phase, thereby ignoring important post-acute infection effects. We present a mathematical model, which not only describes the SARS-CoV-2 infection dynamics during the acute infection phase, but also reflects the recovery of the number of susceptible epithelial cells to an initial pre-infection homeostatic level, shows clearance of the infection within the individual, immune waning, and the formation of long-term immune response levels after infection. Moreover, the model accommodates reinfection events assuming a new virus variant with either increased infectivity or immune escape. Together, the model provides an improved reflection of the SARS-CoV-2 infection dynamics within humans, particularly important when using mathematical models to develop or optimize treatment options.

==> bibliography.tex <==
@article{Ke2022,
    author = "Ke, R. and others",
    title = "{Daily longitudinal sampling of SARS-CoV-2 infection reveals substantial heterogeneity in infectiousness}.",
    journal = "Nature Microbiology",
    volume = "7",
    pages = "640-652",
    year = "2022",
    DOI = "https://doi.org/10.1038/s41564-022-01105-z"
}

@article{Ferretti2020,
    author = "Ferretti L. and others",
    title = "{The timing of COVID-19 transmission}.",
    journal = "medRxiv",
    year = "2020",
    DOI = "https://doi.org/10.1101/2020.09.04.20188516"
}

@article{Szablewski2020,
    author = "Szablewski, C.M. and others",
    title = "{SARS-CoV-2 transmission and infection among attendees of an overnight camp - Georgia, June 2020}.",
    journal = "MMWR Morb Mortal Wkly Rep.",
    volume = "69",
    number={31},
    pages = "1023-1025",
    year = "2020",
    DOI = "http://dx.doi.org/10.15585/mmwr.mm6931e1"
}

@article{Pan2013,
    author = "Pan, Q. and others",
    title = "{Identification of lineage-uncommitted, long-lived, label-retaining cells in healthy human esophagus and stomach, and in metaplastic esophagus}.",
    journal = "Gastroenterology",
    volume = "144",
    number={4},
    pages = "761-770",
    year = "2013",
    DOI = "https://doi.org/10.1053/j.gastro.2012.12.022"
}

@article{Braun2021,
    author = "Braun, K.M. and others",
    title = "{Acute SARS-CoV-2 infections harbor limited within-host diversity and transmit via tight transmission bottlenecks}.",
    journal = "PLOS Pathogens",
    volume = "17",
    number={8},
    year = "2021",
    DOI = "https://doi.org/10.1371/journal.ppat.1009849"
}

@article{Sanche2022,
    author = "Sanche, S. and others",
    title = "{A simple model of COVID‑19
    explains disease severity and the effect of treatments}.",
    journal = "Scientific Reports",
    volume = "12",
    year = "2022",
    DOI = " https://doi.org/10.1038/s41598-022-18244-2"
}

@article{Hernandez-Vargas2020,
    author = "Hernandez-Vargas, E.A. and Velasco-Hernandez, J.X.",
    title = "{In-host mathematical modelling of COVID-19 in humans}.",
    journal = "Annual Reviews in Control",
    volume = "50",
    pages = "448-456",
    year = "2020",
    DOI = "https://doi.org/10.1016/j.arcontrol.2020.09.006"
}

@article{Ke2021,
    author = "Ke, R. and others",
    title = "{In vivo kinetics of SARS-CoV-2 infection and its relationship with a person's infectiousness}.",
    journal = "PNAS",
    volume = "118",
    number={49},
    year = "2021",
    DOI = "https://doi.org/10.1073/pnas.2111477118"
}

@article{Hattaf2023,
    author = "Hattaf, K. and others",
    title = "{Mathematical modeling and analysis of the dynamics of RNA viruses in presence of immunity and treatment: A case study of SARS-Cov-2}.",
    journal = "Vaccines",
    volume = "11",
    number={201},
    year = "2023",
    DOI = "https://doi.org/10.3390/vaccines11020201"
}

@article{Korosec2023,
    author = "Korosec, C.S. and others",
    title = "{Multiple cohort study of hospitalized SARS-CoV-2 in-host infection dynamics: Parameter estimates, identifiability, sensitivity and the eclipse phase profile}.",
    journal = "Journal of Theoretical Biology",
    volume = "564",
    year = "2023",
    DOI = "https://doi.org/10.1016/j.jtbi.2023.111449"
}

@article{Sachak-Patwa2023,
    author = "Sachak-Patwa, R. and others",
    title = "{A target-cell limited model can reproduce influenza infection dynamics in hosts with differing immune responses}.",
    journal = "Journal of Theoretical Biology",
    volume = "567",
    year = "2023",
    DOI = "https://doi.org/10.1016/j.jtbi.2023.111491"
}

@article{Koelle2019,
    author = "Koelle, K. and others",
    title = "{Within-host infectious disease models accommodating cellular coinfection, with an application to influenza}.",
    journal = "Virus Evolution",
    volume = "5",
    number = {2},
    year = "2019",
    DOI = "https://doi.org/10.1093/ve/vez052"
}

@article{Killingley2022,
    author = "Killingley, B. and others",
    title = "{Safety, tolerability and viral kinetics during SARS-CoV-2 human challenge in young adults}.",
    journal = "Nature Medicine",
    volume = "28",
    pages = "1031-1041",
    year = "2022",
    DOI = "https://doi.org/10.1038/s41591-022-01780-9"
}

@article{Puhach2023,
    author = "Puhach, O., and Meyer, B., and Eckerle, I.",
    title = "{SARS-CoV-2 viral load and shedding kinetics}.",
    journal = "Nature Reviews Microbiology",
    volume = "21",
    pages = "147-161",
    year = "2023",
    DOI = "https://doi.org/10.1038/s41579-022-00822-w"
}

@article{Bland1986,
    author = "Bland J.M. and Altman, D.G.",
    title = "{Statistical methods for assessing agreement between two methods of clinical measurement}.",
    journal = "Lancet",
    volume = "327",
    number = {8476},
    pages = "307-310",
    year = "1986",
    DOI = "https://doi.org/10.1016/S0140-6736(86)90837-8"
}

@article{CDC2020,
    author = "National Center for Immunization and Respiratory Diseases (U.S.). Division of Viral Diseases.",
    title = "{Investigative criteria for suspected cases of SARS-CoV-2 reinfection (ICR)}.",
    year = "2020",
    DOI = " https://stacks.cdc.gov/view/cdc/96072"
}

@article{Nguyen2022,
    author = "Nguyen, N.N. and others",
    title = "{SARS-CoV-2 reinfection and COVID-19 severity}.",
    journal = "Emerging Microbes and Infections",
    volume = "11",
    pages = "894-901",
    year = "2022",
    DOI = "https://doi.org/10.1080/22221751.2022.2052358"
}

@article{Diekmann2010,
    author = "Diekmann, O. and Heesterbeek, J.A.P. and Roberts, M.G.",
    title = "{The construction of next-generation matrices for compartmental epidemic models}.",
    journal = "J. R. Soc. Interface",
    volume = "7",
    pages = "873–885",
    year = "2010",
    DOI = "https://doi.org/10.1098/rsif.2009.0386"
}

@article{Ahn2021,
    author = "Ahn, J.H. and others",
    title = "{Nasal ciliated cells are primary targets for SARS-CoV-2 replication in the early stage of COVID-19}.",
    journal = "J. Clin. Invest.",
    volume = "131",
    number = {13},
    year = "2021",
    DOI = "https://doi: 10.1172/JCI148517"
}

@misc{kstest,
year = {2022},
author = {The MathWorks Inc.},
title = {kstest - One-sample Kolmogorov-Smirnov test},
publisher = {The MathWorks Inc.},
address = {Natick, Massachusetts, United States},
url = {https://it.mathworks.com/help/stats/kstest.html}
}

@article{Ghosh2020,
    author = "Ghosh, S. and others",
    title = "{$\beta$-Coronaviruses sse lysosomes for egress instead of the biosynthetic secretory pathway}.",
    journal = "Cell",
    volume = "183",
    pages = "1520–1535",
    year = "2020",
    DOI = "https://doi.org/10.1016/j.cell.2020.10.039"
}

@misc{kstest2,
year = {2022},
author = {The MathWorks Inc.},
title = {kstest2 - Two-sample Kolmogorov-Smirnov test},
publisher = {The MathWorks Inc.},
address = {Natick, Massachusetts, United States},
url = {https://it.mathworks.com/help/stats/kstest2.html}
}

@article{Armstrong2014,
    author = "Armstrong, R.A.",
    title = "{When to use the Bonferroni correction}.",
    journal = "Ophthalmic and Physiological Optics",
    volume = "34",
    number = {5},
    pages = "502 - 508",
    year = "2014",
    DOI = "https://doi.org/10.1111/opo.12131"
}

@article{Hass2019,
    author = "Hass, H. and others",
    title = "{Benchmark problems for dynamic modeling of intracellular processes}.",
    journal = "Bioinformatics",
    volume = "35",
    number = {17},
    pages = "3073–3082",
    year = "2019",
    DOI = "https://doi.org/10.1093/bioinformatics/btz020"
}

@article{Ruysseveldt2021,
    author = "Ruysseveldt, E. and others",
    title = "{Airway basal cells, protectors of epithelial walls in health and respiratory diseases}.",
    journal = "Front. Allergy",
    volume = "2",
    year = "2021",
    DOI = "https://doi.org/10.3389/falgy.2021.787128"
}

@article{Phan2023,
    author = "Phan, T. and others",
    title = "{Modeling the emergence of ciral resistance for SARS-CoV-2 during treatment with anti-spike monoclonal antibody}.",
    journal = "bioRxiv",
    year = "2023",
    DOI = "https://doi.org/10.1101/2023.09.14.557679"
}

@article{Marc2023,
    author = "Marc, A. and others",
    title = "{Impact of variants of concern on SARS-CoV-2 viral dynamics in non-human primates}.",
    journal = "PLOS Computational Biology",
    volume = "19",
    number = {8},
    year = "2023",
    DOI = "https://doi.org/10.1371/journal.pcbi.1010721"
}

@article{Cox2020,
    author = "Cox, R.J. and Brokstad, K.A.",
    title = "{Not just antibodies: B cells and T cells mediate immunity to COVID-19}.",
    journal = "Nature Reviews Immunology",
    volume = "20",
    pages = "581-582",
    year = "2020",
    DOI = "https://doi.org/10.1038/s41577-020-00436-4"
}

@article{Sette2021,
    author = "Sette, A. and Crotty, S.",
    title = "{Adaptive immunity to SARS-CoV-2 and COVID-19}.",
    journal = "Cell",
    volume = "184",
    pages = "861-880",
    year = "2021",
    DOI = "https://doi.org/10.1016/j.cell.2021.01.007"
}

@article{Rodda2021,
    author = "Rodda, L.B. and others",
    title = "{Functional SARS-CoV-2-specific immune memory persists after mild COVID-19}.",
    journal = "Cell",
    volume = "184",
    pages = "169-183",
    year = "2021",
    DOI = "https://doi.org/10.1016/j.cell.2020.11.029"
}

@article{Yang2023,
    author = "Yang, Y. and others",
    title = "{Viral and antibody dynamics of acute infection with SARS-CoV-2 omicron variant (B.1.1.529): a prospective cohort study from Shenzhen, China}.",
    journal = "Lancet Microbe",
    volume = "4",
    pages = "e632-e641",
    year = "2023",
    DOI = "https://doi.org/10.1016/S2666-5247(23)00139-8"
}

@article{Marc2021,
    author = "Marc, A. and others",
    title = "{Quantifying the relationship between SARS-CoV-2 viral load and infectiousness}.",
    journal = "eLife",
    year = "2021",
    DOI = "https://doi.org/10.7554/eLife.69302"
}

@article{Wang2020,
    author = "Wang, S. and others",
    title = "{Modeling the viral dynamics of SARS-CoV-2 infection}.",
    journal = "Mathematical Biosciences",
    volume = "328",
    year = "2020",
    DOI = "https://doi.org/10.1016/j.mbs.2020.108438"
}

@article{Challenger2022,
    author = "Challenger, J.D. and others",
    title = "{Modelling upper respiratory viral load dynamics of SARS-CoV-2}.",
    journal = "BMC Medicine",
    volume = "20",
    year = "2022",
    DOI = "https://doi.org/10.1186/s12916-021-02220-0"
}

@article{McCormack2023,
    author = "McCormack, C.P. and others",
    title = "{Modelling the viral dynamics of the SARS-CoV-2 Delta and Omicron variants in different cell types}.",
    journal = "J. R. Soc. Interface",
    volume = "20",
    year = "2023",
    DOI = "https://doi.org/10.1098/rsif.2023.0187"
}


@article{Canini2014,
    author = "Canini, L. and Perelson, A.S.",
    title = "{Viral kinetic modeling: state of the art}.",
    journal = "J Pharmacokinet Pharmacodyn",
    volume = "41",
    number = {5},
    pages = "431-443",
    year = "2014",
    DOI = "https://doi.org/10.1007\%2Fs10928-014-9363-3"
}

@article{Perelson2023,
    author = "Perelson, A.S. and Ribeiro, R.M. and Phan, T.",
    title = "{An axplanation for SARS-CoV-2 rebound after Paxlovid treatment}.",
    journal = "medRxiv",
    year = "2023",
    DOI = "https://doi.org/10.1101/2023.05.30.23290747"
}

@article{Phan2023,
    author = "Phan, T. and others",
    title = "{Modeling the emergence of viral resistance for SARS-CoV-2 during treatment with an anti-spike monoclonal antibody}.",
    journal = "bioRxiv",
    year = "2023",
    DOI = "https://doi.org/10.1101/2023.09.14.557679"
}

@article{Choudhary2022,
    author = "Choudhary, M.C. and others",
    title = "{Emergence of SARS-CoV-2 escape mutations duringmBamlanivimab therapy in a phase II randomized clinical trial}.",
    journal = "Nature Microbiology",
    volume = "7",
    year = "2022",
    DOI = "https://doi.org/10.1038/s41564-022-01254-1"
}

@article{Woelfel2020,
    author = "Woelfel, R. and others",
    title = "{Virological assessment of hospitalized patients with COVID-2019}.",
    journal = "Nature",
    volume = "581",
    pages = "465–469",
    year = "2020",
    DOI = "https://doi.org/10.1038/s41586-020-2196-x"
}

@book{Kuznetsov1998,
  title     = "Elements of Applied Bifurcation Theory",
  author    = "Yuri A. Kuznetsov",
  year      = 1998,
  publisher = "Springer",
  address   = "New York"
}

@article{BarOn2020,
    author = "Bar-On, Y.M. and others",
    title = "{Science Forum: SARS-CoV-2 (COVID-19) by the numbers}.",
    journal = "eLife",
    volume = "9",
    year = "2020",
    DOI = "https://doi.org/10.7554/eLife.57309"
}

@article{Sender2021,
    author = "Sender, R. and others",
    title = "{The total number and mass of SARS-CoV-2 virions}.",
    journal = "PNAS",
    volume = "118",
    number = {25},
    year = "2021",
    DOI = "https://doi.org/10.1073/pnas.2024815118"
}

@article{Du2022,
    author = "Du, Z. and others",
    title = "{Within-host dynamics of SARS-CoV-2 infection: A systematic review and meta-analysis}.",
    journal = "Transboundary and Emerging Diseases",
    volume = "69",
    pages = "3964-3971",
    year = "2022",
    DOI = "https://doi.org/10.1111/tbed.14673"
}

@article{Kissler2023,
    author = "Kissler, S.M. and others",
    title = "{Viral kinetics of sequential SARS-CoV-2 infections}.",
    journal = "Nature Communications",
    volume = "14",
    year = "2023",
    DOI = "https://doi.org/10.1038/s41467-023-41941-z"
}

@article{Du2020,
    author = "Du, X. and others",
    title = "{Duration for carrying SARS-CoV-2 in COVID-19 patients}.",
    journal = "Journal of Infection",
    volume = "81",
    number = {1},
    year = "2020",
    DOI = "https://doi.org/10.1016/j.jinf.2020.03.053"
}

@article{Goncalves2020,
    author = "Gon\c{c}alves, A. and others",
    title = "{Timing of antiviral treatment initiation is critical to reduce SARS-CoV-2 viral load}.",
    journal = "CPT Pharmacometrics Syst. Pharmacol.",
    volume = "9",
    pages = "509-514",
    year = "2020",
    DOI = "https://doi.org/10.1002/psp4.12543"
}
